Correction methods for finite-acceptance effects in two-particle correlation analyses

Two-particle angular correlations have been widely used as a tool to explore particle production mechanisms in heavy-ion collisions. The mixed-event technique is generally used as a standard method to correct for finite-acceptance effects. We demonstrate that event mixing only provides an approximate acceptance correction, and propose new methods for finite-acceptance corrections. Starting from discussions about 2-dimensional correction procedures, new methods are derived for specific assumptions on the properties of the signal, such as uniform signal distribution or $\delta$-function-like trigger particle distribution, and suitable for two-particle correlation analyses from particles at mid-rapidity and jet-hadron or high $p_{\text{T}}$-triggered hadron-hadron correlations. Per-trigger associated particle yields from the mixed-event method and the new methods are compared through Monte Carlo simulations containing well-defined correlation signals. Significant differences are observed at large pseudorapidity differences in general and especially for asymmetric particle distribution like that produced in proton--nucleus collisions. The applicability and validity of the new methods are discussed in detail.

==> Makefile <==
#############################


TEXSDIR   = ./
PICSDIR   = ./img
FILENAME  = NewMethod

###

TEXSRCS   = $(shell find $(TEXSDIR) -maxdepth 1 -iname "*.tex")
PICS      = $(shell find $(PICSDIR) -maxdepth 1 -iname "*.eps")

ADDFILES  = Makefile

BACKFILES = $(PICS) $(TEXSRCS) 

ARCHFILES = $(TEXSRCS) \

SENDFILES = $(TEXSRCS)

PDFPICS   = $(patsubst %.eps,%.pdf,$(PICS))

LATEX	  = latex
PDFTEX    = pdflatex
DVIPS	  = dvips
PS2PDF    = ps2pdf
EPS2EPS   = eps2eps
EPSTOPDF  = epstopdf
THUMBPDF  = thumbpdf
BIBTEX    = bibtex
#EPSOPTION = --hires 

default:	$(FILENAME).pdf

$(FILENAME):		$(FILENAME).dvi

$(FILENAME).pdf:	$(FILENAME).tex $(TEXSRCS) $(ADDFILES) $(PDFPICS) 
	$(PDFTEX) 	$(FILENAME)
	$(BIBTEX)       $(FILENAME)
	$(PDFTEX) 	$(FILENAME)
	$(PDFTEX) 	$(FILENAME)

$(FILENAME).dvi:	$(FILENAME).tex $(TEXSRCS) $(ADDFILES)
	$(LATEX) 	$(FILENAME)
	$(BIBTEX)       $(FILENAME)
	$(LATEX) 	$(FILENAME)
	$(LATEX) 	$(FILENAME)

$(FILENAME).ps:		$(FILENAME).dvi $(PICS)
	$(DVIPS) $(FILENAME).dvi -o $(FILENAME).ps


$(FILENAME).tar.gz:	backup

dvi:	$(FILENAME).dvi

ps:	$(FILENAME).ps

gzip:	ps
	gzip $(FILENAME).ps

pdf:	$(FILENAME).pdf

ps2pdf:	$(FILENAME).dvi
	$(DVIPS) -Ppdf $(FILENAME).dvi -o $(FILENAME).ps
	$(PS2PDF) $(FILENAME).ps

print:  $(FILENAME).ps
	lpr $(FILENAME).ps

vdvi:	$(FILENAME).dvi
	xdvi $(FILENAME).dvi &

vps:	$(FILENAME).ps
	gv $(FILENAME).ps &

vpdf:	$(FILENAME).pdf
	evince $(FILENAME).pdf &

edit:
	emacs $(FILENAME).tex

clean:
	rm -f $(FILENAME).dvi $(FILENAME).toc .tmp.eps	\
	$(FILENAME).aux $(FILENAME).out $(FILENAME).tpt \
	$(FILENAME).bbl $(FILENAME).blg $(FILENAME).log \
	$(FILENAME).lof $(FILENAME).lot $(FILENAME).idx \
	$(FILENAME).ind $(FILENAME).ilg $(FILENAME).glo \
	$(FILENAME).blg $(FILENAME).brf missfont.log \
        texput.log core *.aux *.tmp
	find $(TEXSDIR) $(PICSDIR) -name "*~" -type f -exec rm -f "{}" \;
	find $(TEXSDIR) $(PICSDIR) -type d -exec chmod 755 "{}" \;
	find $(TEXSDIR) $(PICSDIR) -type f -exec chmod 644 "{}" \;
	find $(TEXSDIR) -name "*.sh" -type f -exec chmod 755 "{}" \;

realclean: clean
	rm -f $(FILENAME).ps.gz $(FILENAME).pdf $(PDFPICS) $(FILENAME).ps $(FILENAME).tar.gz archiv.tar.gz

archiv:
	echo $(ARCHFILES)
	tar -cvzf archiv.tar.gz $(FILENAME).tex $(ARCHFILES)

backup:
	tar -cvzf $(FILENAME).tar.gz $(FILENAME).tex $(BACKFILES) $(ADDFILES)

.phony: print clean backup

$(PDFPICS): %.pdf: %.eps
	$(EPS2EPS) $< .tmp.eps && $(EPSTOPDF) $(EPSOPTION) .tmp.eps --outfile=$@ && rm -f .tmp.eps

